Monte Carlo Filtering Objectives: A New Family of Variational Objectives to Learn Generative Model and Neural Adaptive Proposal for Time Series

Learning generative models and inferring latent trajectories have shown to be challenging for time series due to the intractable marginal likelihoods of flexible generative models. It can be addressed by surrogate objectives for optimization. We propose Monte Carlo filtering objectives (MCFOs), a family of variational objectives for jointly learning parametric generative models and amortized adaptive importance proposals of time series. MCFOs extend the choices of likelihood estimators beyond Sequential Monte Carlo in state-of-the-art objectives, possess important properties revealing the factors for the tightness of objectives, and allow for less biased and variant gradient estimates. We demonstrate that the proposed MCFOs and gradient estimations lead to efficient and stable model learning, and learned generative models well explain data and importance proposals are more sample efficient on various kinds of time series data.

==> boarderimpact.tex <==
%Authors are required to include a statement of the broader impact of their work, including its ethical aspects and future societal consequences. Authors should discuss both positive and negative outcomes, if any. For instance, authors should discuss a) who may benefit from this research, b) who may be put at disadvantage from this research, c) what are the consequences of failure of the system, and d) whether the task/method leverages biases in the data. If authors believe this is not applicable to them, authors can simply state this.

With much recent progress in learning generative models on non-sequential data, inference and learning models of time series remain challenging due to its complex nature. We hope our study would provide some insights into generalized surrogate objectives to learn generative and amortized proposal models for time series, and provide guidance to explore a wider set of sampling methods to improve learning and learned models. 

We believe our study could benefit on filtering problems and modeling of complex time series, and their broad applications e.g. object tracking, dynamical system identification, time series prediction in finance and other areas. Potential disadvantages are more related to the particular use case rather than to the proposed methods.

At this stage of study, we cannot foresee the effects of potential system failures due to weaknesses in the proposed methods. However, we would like to point out that for challenging time series data such as those with high signal-to-noise ratios, no underlying patterns or long time dependency, it is not so clear whether learning is possible and whether the method would work.

==> method.tex <==
\iffalse
In this section, we propose MCFOs, a family of variational filtering objectives, inspired by MCOs and FIVOs. We examine their important properties and discuss the choice of importance proposal on the tightness of MCFOs and their relations to previous objectives and how to optimize MCFOs to learn parametric generative and adaptive proposal models from data.
\fi
%\subsection{Definition and Properties}
The key to efficiently compute a maximum likelihood estimate of time series generative models is to decompose the joint marginal log-likelihood by:\vspace{-2mm}
\begin{equation}
    \log p(\mathbf{x}_{1:T}) = \log p(\mathbf{x}_1) + \sum_{t=2}^T \log p(\mathbf{x}_t|\mathbf{x}_{1:t-1}),
    \label{eq:recursion}
\end{equation}
such that each $\log p(\mathbf{x}_t|\mathbf{x}_{1:t-1})$ can be computed recursively. Nonetheless, the conditional marginal log-likelihoods in (\ref{eq:recursion}) are usually intractable, which means that direct maximization of the marginal, for learning a generative sequence model, is possible only in limited cases.% of arbitrary length.
%where the marginal likelihood $Z_t := p(\mathbf{x}_{1:t})$. Instead of using unbiased estimator by SMC to define lower bound on whole trajectory $p(\mathbf{x}_{1:T})$ as AESMC/VSMC/FIVO, 

We thus define an MCO, $\mathcal{L}_t^K$, to estimate the intractable $\log p(\mathbf{x}_t|\mathbf{x}_{1:t-1})$ with $K$ samples: %\vspace{-1mm}
\begin{equation}
\begin{aligned}
    &  \mathcal{L}_t^K = %\mathbb{E}_{Q_t^K}\left[
    %{p(\mathbf{z}_{1:t-1}^{i}|\mathbf{x}_{1:t-1}) q(\mathbf{z}_{t}^{i}|\mathbf{z}_{1:t-1}^{i},\mathbf{x}_{1:t})} 
    %\log \left( \frac{1}{K} \sum_{i=1}^K \frac{p(\mathbf{z}_{1:t}^{i},\mathbf{x}_{1:t})}{p(\mathbf{z}_{1:t-1}^{i},\mathbf{x}_{1:t-1})q(\mathbf{z}_{t}^{i}|\mathbf{z}_{1:t-1}^{i},\mathbf{x}_{1:t})} \right) \right],
    \mathbb{E}_{Q_t^K}[\log R_t^K], \\ 
    & Q_t^K%(\mathbf{z}_{1:t}^{1:K}, \mathbf{x}_{1:t})
        = p(\mathbf{z}_{1:t-1}^{1:K}|\mathbf{x}_{1:t-1}) \cdot \prod_{i=1}^K  q(\mathbf{z}_{t}^{i}|\mathbf{z}_{1:t-1}^{i},\mathbf{x}_{1:t}), \\
    & R_t^K%(\mathbf{z}_{1:t}^{1:K}, \mathbf{x}_{1:t})
        = \frac{1}{K} \sum_{i=1}^K \frac{p(\mathbf{z}_{1:t}^{i},\mathbf{x}_{1:t})}{p(\mathbf{z}_{1:t-1}^{i},\mathbf{x}_{1:t-1})q(\mathbf{z}_{t}^{i}|\mathbf{z}_{1:t-1}^{i},\mathbf{x}_{1:t})},
\end{aligned}
\label{eq:L_t_k}
\end{equation}
specifically $\mathcal{L}_1^K$ for $\log p(\mathbf{x}_1)$, \vspace{-1mm}
\begin{equation}
\begin{aligned}
    & Q_1^K%(\mathbf{z}_{1}^{1:K}, \mathbf{x}_{1})
        = \prod_{i=1}^K q(\mathbf{z}_1^{i}|\mathbf{x}_1), ~~
        R_1^K%(\mathbf{z}_{1}^{1:K}, \mathbf{x}_{1})
        = \frac{1}{K} \sum_{i=1}^K \frac{p(\mathbf{z}_1^{i}, \mathbf{x}_1)}{q(\mathbf{z}_1^{i}|\mathbf{x}_1)},
\end{aligned}
%\label{eq:L_t_k}
\nonumber
\end{equation}
where %$Q_t^K$ %= {p(\mathbf{z}_{1:t-1}|\mathbf{x}_{1:t-1}) q(\mathbf{z}_{t}|\mathbf{z}_{1:t-1},\mathbf{x}_{1:t})}$ is the proposal distribution of the joint posterior $p(\mathbf{z}_{1:t}|\mathbf{x}_{1:t})$, and
$q(\mathbf{z}_{t}|\mathbf{z}_{1:t-1},\mathbf{x}_{1:t})$ and $q(\mathbf{z}_{1}|\mathbf{x}_{1:t})$ are the proposal distribution% of $p(\mathbf{z}_{t}|\mathbf{z}_{1:t-1},\mathbf{x}_{1:t})$
, $R_t^K$ and $R_1^K$ are estimators of conditional marginal $p(\mathbf{x}_{t}|\mathbf{x}_{1:t-1})$ and $p(\mathbf{x}_{1})$; see Appendix \ref{sec:appendix_lower_bound} for a more detailed derivation. Using the recursion in (\ref{eq:recursion}), we then define a Monte Carlo filtering objective (MCFO), $\mathcal{L}_{\text{MCFO}}$, by summing a series of MCOs defined in (\ref{eq:L_t_k}):\vspace{-1mm}
\begin{equation}
    \begin{aligned}
        & \log p(\mathbf{x}_{1:T}) 
        \geq \mathcal{L}_{\text{MCFO}}^K (\mathbf{x}_{1:T}, p, q) %\\
        %& \quad \quad \quad \quad \quad \quad 
        = \sum_{t=1}^T \mathcal{L}_t^K. %= \sum_{t=1}^T \mathbb{E}_{Q_t^K}[\log R_t^K],\\
        %& Q_1^K%(\mathbf{z}_{1}^{1:K}, \mathbf{x}_{1}) = \prod_{i=1}^K q(\mathbf{z}_1^{i}|\mathbf{x}_1), %R_1^K%(\mathbf{z}_{1}^{1:K}, \mathbf{x}_{1}) = \frac{1}{K} \sum_{i=1}^K \frac{p(\mathbf{z}_1^{i}, \mathbf{x}_1)}{q(\mathbf{z}_1^{i}|\mathbf{x}_1)},
        \\ 
        %& Q_t^K%(\mathbf{z}_{1:t}^{1:K}, \mathbf{x}_{1:t}) = p(\mathbf{z}_{1:t-1}^{1:K}|\mathbf{x}_{1:t-1}) \cdot \prod_{i=1}^K  q(\mathbf{z}_{t}^{i}|\mathbf{z}_{1:t-1}^{i},\mathbf{x}_{1:t}). \\
        %& R_t^K%(\mathbf{z}_{1:t}^{1:K}, \mathbf{x}_{1:t})
        %= \frac{1}{K} \sum_{i=1}^K \frac{p(\mathbf{z}_{1:t}^{i},\mathbf{x}_{1:t})}{p(\mathbf{z}_{1:t-1}^{i},\mathbf{x}_{1:t-1})q(\mathbf{z}_{t}^{i}|\mathbf{z}_{1:t-1}^{i},\mathbf{x}_{1:t})}.
    \end{aligned} 
\end{equation}
To avoid notation clutter, we leave out arguments on $\mathcal{L}_{\text{MCFO}}^K$, $Q_t^K$ and $R_t^K$ where context permits. Except for some general properties inherited from MCOs such as \textit{bound} and \textit{consistency} \citep{maddison2017filtering}, the convergence of MCFOs to $\log p(\mathbf{x}_{1:T})$ is \textit{monotonic} like IW-ELBO \citep{burda2015importance}, but different from FIVOs, AESMC and VSMC. Additionally, by extending \citep[Theorem~3]{domke2018importance}, we can obtain the asymptotic bias of MCFOs that relates to the total variances of the series of estimators. %\vspace{-1mm}
\begin{proposition}
\label{prop:properties}
(\textnormal{Properties of MCFOs}). Let $\mathcal{L}_{\text{MCFO}}^K$ be an MCFO of $\log p(\mathbf{x}_{1:T}) $ by a series of unbiased estimators $R_t$ of $p(\mathbf{x}_t|\mathbf{x}_{1:t-1})$ using $K$ samples. Then, 
\begin{enumerate}[label=\alph*)] % (a), (b), (c), ...
\item \label{prop:properties_1} \textnormal{(Bound)} $\log p(\mathbf{x}_{1:T}) \geq \mathcal{L}_{\text{MCFO}}^K$.
\item \label{prop:properties_2} \textnormal{(Monotonic convergence)} $\mathcal{L}_{\text{MCFO}}^{K+1} \geq \mathcal{L}_{\text{MCFO}}^{K} \geq  \hdots \geq  \mathcal{L}_{\text{MCFO}}^{1}$.
\item \label{prop:properties_3} \textnormal{(Consistency)} if $p(\mathbf{z}_{1},\mathbf{x}_{1}) /q(\mathbf{z}_{1}|\mathbf{x}_{1})$ and ${p(\mathbf{z}_{1:t},\mathbf{x}_{1:t})}/{(p(\mathbf{z}_{1:t-1},\mathbf{x}_{1:t-1})q(\mathbf{z}_{t}|\mathbf{z}_{1:t-1},\mathbf{x}_{1:t}))}$ for all $t\in[2,T]$ are bounded, then $\mathcal{L}_{\text{MCFO}}^K \rightarrow \log p(\mathbf{x}_{1:T})$ as K $\rightarrow \infty$.
\item \label{prop:properties_4} \textnormal{(Asymptotic Bias)} For a large K, the bias of bound is related to the variance of estimator $R_t$, $\mathbb{V}[R_t]$, 
\[\lim_{K\rightarrow \infty} K(\log p(\mathbf{x}_{1:T}) - \mathcal{L}_{\text{MCFO}}^K) = \sum_{t=1}^T \frac{\mathbb{V}[R_t]}{2 p(\mathbf{x}_t|\mathbf{x}_{1:t-1})^2}. \]
\end{enumerate}
\end{proposition}
\textit{Proof.} See Appendix \ref{sec:appendix_lower_bound_property}.

As shown by \textit{monotonic convergence} and \textit{asymptotic bias}, increasing the number of samples and using lower variant estimators $R_t$ lead to a tighter MCFO. Theoretically, an unlimited number of samples gives the exact estimate of the marginal log-likelihood. Since this is not feasible in practice, the number can instead be chosen based on available computational resources. %Nevertheless, it is impossible and inefficient in practice, and it can be chosen according to computational resources. 
Additionally, although resampling introduces extra intermediate variance, it helps to lower the total variance and therefore makes the bound tighter.

% SMC would outperform with SIS, as resampling in SMC reduces the variance sum of estimators. %This makes SMC and other Monte Carlo Markov Chain (MCMC) methods preferred over SIS for tighter bounds. %To be noted, the asymptotic bias only applies when K is adequately large so it might not always apply at small K regime \citet{rainforth2018tighter}.


Considering the filtering problem, that assumes that future observations have no impact on the posterior, replacing $p(\mathbf{z}_{1:t-1}^{1:K}|\mathbf{x}_{1:t-1})$ in $Q_t^K(\mathbf{z}_{1:t}^{1:K}|\mathbf{x}_{1:t})$ by K sample approximation $\hat{p}(\mathbf{z}_{1:t-1}^{1:K}|\mathbf{x}_{1:t-1}) = \sum_{i=1}^K \Tilde{w}_{t-1}^{i} \delta(\mathbf{z}_{1:t-1}^{1:K}-\hat{\mathbf{z}}_{1:t-1}^{1:K})$ leads to the definition of FIVOs. %(where $\hat{\mathbf{z}}_{1:t}^{1:K}$ are sample trajectories before resampling step in SMC) 
With this approximation, FIVOs could be considered as a biased estimate of MCFOs using SMC sampling. They are consistent to MCFOs and the asymptotic bias is $\mathcal{O}(1/K)$; see detailed discussion and proof in Appendix \ref{sec:fivo_and_mcfo}. Although MCFOs are commonly intractable and cannot be unbiasedly estimated when using SMC-like estimators, they are tractable and practical e.g. using the posterior reparameterized by normalizing flows \citep{rezende2015variational}. MCFOs extend sampling methods to more alternatives, such as PIMH \citep{andrieu2010particle} and unbiased MCMC with couplings \citep{jacob2017unbiased} to further improve sample efficiency and scale to high dimensional problems. Later, we show that MCFOs facilitate the implementation of less biased and variant gradient estimators, which lead to faster and more stable learning of generative and proposal models.


\subsection{Importance proposals}
\label{sec:importance_proposal}

Asymptotic bias shows that the tightness of MCFOs is dependent on the variance of estimators (or, equivalently the variance of importance weights), and the variance of estimators is determined by the choice of importance proposals. Therefore, a poor proposal leads to poor sample efficiency, a weak approximation of true posterior, and higher variance of estimates. Some negative effects could be mitigated by increasing the number of samples and/or applying additional MCMC moves \citep{doucet2009tutorial} but at a computational cost. Therefore, appropriate proposals, learned or designed, are key instruments for MCFOs. Considering $q$ as an argument of MCFOs, we can derive the optimal proposal. %by maximizing MCFOs.
\begin{proposition}
\textnormal{Optimal importance proposal $q^*$ for an MCFO}. The bound is maximized and exact to $\log p(\mathbf{x}_{1:T})$ when the optimal importance proposals are
\begin{equation*}
    \begin{aligned}
        & q^*(\mathbf{z}_{1}|\mathbf{x}_{1}) = p(\mathbf{z}_{1}|\mathbf{x}_{1}), \\
        & q^*(\mathbf{z}_{t}|\mathbf{z}_{1:t-1},\mathbf{x}_{1:t}) = p(\mathbf{z}_{t}|\mathbf{z}_{1:t-1}, \mathbf{x}_{1:t}) = \frac{p(\mathbf{z}_{1:t}|\mathbf{x}_{1:t})}{p(\mathbf{z}_{1:t-1}|\mathbf{x}_{1:t-1})},\\
        & \text{for all } t=2:T.\\
    \end{aligned}
\end{equation*}
\end{proposition}
\textit{Proof.} See Appendix A.3.

The optimal importance proposals always aim to move samples from the previous target posterior $p(\mathbf{z}_{1:t-1}|\mathbf{x}_{1:t-1})$ to the new target posterior $p(\mathbf{z}_{1:t}|\mathbf{x}_{1:t})$. These optimal proposals minimize the variance of all estimators to 0 so that MCFOs become exact to the marginal log-likelihood. For SSMs that assume latent variables with Markovian property, $p(\mathbf{z}_{t}| \mathbf{z}_{1:t-1})=p(\mathbf{z}_{t}|\mathbf{z}_{t-1}), p(\mathbf{z}_{t-1}|\mathbf{z}_{t:T}, \mathbf{x}_{t:T})=p(\mathbf{z}_{t}|\mathbf{z}_{t-1})$, and conditional independence on observations, $p(\mathbf{x}_{t}|\mathbf{z}_{1:t},\mathbf{x}_{1:t-1})  = p(\mathbf{x}_{t}|\mathbf{z}_{t})$ \citep{sarkka2013bayesian}, the optimal importance proposal is further simplified to $p(\mathbf{z}_{t}|\mathbf{z}_{t-1}, \mathbf{x}_{t}), \text{for all } t=2:T$ as \citep[Proposition~2]{doucet2000sequential}. However, in practice, we have no access to the true posteriors, $p(\mathbf{z}_{1}|\mathbf{x}_{1})$ or $p(\mathbf{z}_{1:t}|\mathbf{x}_{1:t})$ or $p(\mathbf{z}_{1:t-1}|\mathbf{x}_{1:t-1})$. We thus aim to learn the adaptive importance proposals by maximizing MCFOs, jointly with a generative model. 

\subsection{Optimization}
\label{sec:gradient_estimate}

One of the goals of an MCFO is to learn flexible parametric proposals and/or generative models by optimization. The proposed method could be applied to any parametric distribution, where we explicitly parameterize the generative models $p_{\boldtheta}$ by $\boldtheta$ and the importance proposal models $q_{\boldphi}$ by $\boldphi$ respectively. %Although EM algorithm could maximize tractable MCFOs, however, i
In practice, gradient ascent algorithms using Monte Carlo gradient estimates 
have been found to be flexible when optimizing 
%is found more flexible to optimize any
differentiable parametric distributions. 

The gradients of an MCFO with respect to $\boldtheta$ and $\boldphi$, are decomposed as $\triangledown_{\boldtheta, \boldphi} \mathcal{L}_{\text{MCFO}}^K = \sum_{t=1}^T \triangledown_{\boldtheta, \boldphi} \mathcal{L}_t^K$, and each $\triangledown_{\boldtheta, \boldphi} \mathcal{L}_t^K $ can be further specified by two terms, $\mathbb{E}_{Q_t^K}\left[\log R_t^K \triangledown_{\boldtheta, \boldphi} \log Q_t^K \right]$ and $\mathbb{E}_{Q_t^K}\left[ \triangledown_{\boldtheta, \boldphi} \log R_t^K  \right]$; see Appendix \ref{sec:appendix_gradient_theta} for detailed derivations. The first term dominates the variance in the gradient estimate mainly due to 1) large magnitudes of $\log R_t^K$ especially at the beginning of training \citep{mnih2014neural}; 2) high variance from the discrete variables for ancestral index of resampling in SMC \citep{naesseth2018variational, le2017auto, maddison2017filtering}. To lower the variance to stabilize learning, earlier methods ignore the dominant high variance term. This, however, comes at the cost of an additional bias that cannot be eliminated by increasing the number of samples, and potentially deteriorates the convergence of parameter learning \citep{roeder2017sticking}. 

MCFOs circumvent the high variance in gradient estimates of $\triangledown_{\boldphi} \mathcal{L}_{\text{MCFO}}^K $ without the extra bias. Assuming the proposal distribution $q_{\boldphi}$ is reparameterizable \citep{mohamed2019monte}, $\triangledown_{\boldphi} \mathcal{L}_t^K$ could be estimated with less variance using \textit{reparameterization trick} by:
\begin{equation}
    \begin{aligned}
        \triangledown_{\boldphi} \mathcal{L}_t^K & = \mathbb{E}_{p_{\boldtheta}(\mathbf{z}_{1:t-1}^{i}|\mathbf{x}_{1:t-1})} [\triangledown_{\boldphi} \mathbb{E}_{q_{\boldphi}(\mathbf{z}_{t}^{i}|\mathbf{z}_{1:t-1}^{i},\mathbf{x}_{1:t})}
        [\log \frac{1}{K} \sum_{i=1}^K %\frac{p(\mathbf{x}_{t}|\mathbf{z}_{1:t}^{i},\mathbf{x}_{1:t-1}^{i})p(\mathbf{z}_{t}^{i}|\mathbf{z}_{1:t-1}^{i}, \mathbf{x}_{1:t-1}^{i})}{q_{\boldphi}(\mathbf{z}_{t}^{i}|\mathbf{z}_{1:t-1}^{i},\mathbf{x}_{1:t})}]]\\
        \frac{p_{\boldtheta}(\mathbf{z}_{1:t}^{i},\mathbf{x}_{1:t})}{p_{\boldtheta}(\mathbf{z}_{1:t-1}^{i},\mathbf{x}_{1:t-1})q_{\boldphi}(\mathbf{z}_{t}^{i}|\mathbf{z}_{1:t-1}^{i},\mathbf{x}_{1:t})}]]\\
        \simeq & \triangledown_{\boldphi}f_{\boldtheta,\boldphi}(\mathbf{x}_{1:t},\hat{\mathbf{z}}_{1:t-1}^{1:K}, 
        \underbrace{ g_{\boldphi}(\hat{\mathbf{z}}_{1:t-1}^{1}, \boldsymbol{\epsilon}^i, \mathbf{x}_{1:t}), \hdots, g_{\boldphi}(\hat{\mathbf{z}}_{1:t-1}^{K},\boldsymbol{\epsilon}^K, \mathbf{x}_{1:t})}_{\text{reparameterization trick, } \hat{\mathbf{z}}_{t}^{i} = g_{\boldphi}(\hat{\mathbf{z}}_{1:t-1}^{i}, \mathbf{x}_{1:t}, \boldsymbol{\epsilon}^i)}), 
        % \log \frac{1}{K} \sum_{i=1}^K  \frac{p(g_{\phi}^{i}(\mathbf{z}_{t-1}^{i},\epsilon, \mathbf{x}_t)|\mathbf{x}_{t})p(g_{\phi}^{i}(\mathbf{z}_{t-1}^{i},\epsilon, \mathbf{x}_t)|\mathbf{z}_{t-1}^{i})}{q_{\boldphi}(g_{\phi}^{i}(\mathbf{z}_{t-1}^{i},\epsilon, \mathbf{x}_t)|\mathbf{z}_{t-1}^{i},\mathbf{x}_{t})}]
    \end{aligned}
    \label{eq:gradient_phi}
\end{equation}
where $f_{\boldtheta,\boldphi}(\cdot)$ is the logarithm average function $\log \frac{1}{K} \sum_{i=1}^K \left( \frac{\cdot}{\cdot} \right)$, and $\boldsymbol{\epsilon}^i \sim p(\boldsymbol{\epsilon})$. %To be noted, the only resource of biasness of this gradient is from posterior approximation $\hat{p}_{\boldtheta}(\mathbf{z}_{1:t-1}|\mathbf{x}_{1:t-1})$ to true posterior $p_{\boldtheta}(\mathbf{z}_{1:t-1}|\mathbf{x}_{1:t-1})$. 
% To be noted, the inner expectation 
%if $f_{\boldtheta,\boldphi}(\cdot)$ is assumed differentiable, while the estimates by score function are biased \citep{mohamed2019monte}. Thus when generative parameters also converge and samples from $p_{\boldtheta}(\mathbf{z}_{1:t-1}|\mathbf{x}_{1:t-1})$ are distributed as $p(\mathbf{z}_{1:t-1}|\mathbf{x}_{1:t-1})$, the gradient $\triangledown_{\boldphi} \mathcal{L}_t^K$ would become unbiased and have 0 mean at its optimum.

%Different from the variance explosion in the original AESMC, VSMC and FIVOs, decomposing the global estimator into multiple local estimators is a way of Rao-Blackwellization to reduce variance in the gradient. Although samples $\mathbf{z}_{1:t-1}^{1:K}$ are indirectly dependent on $\boldphi$ through proposals, the posterior $p_{\boldtheta}(\mathbf{z}_{1:t-1}|\mathbf{x}_{1:t-1})$ is only conditioned on generative parameters $\boldtheta$. Therefore, we can decouple the first expectation over $p_{\boldtheta}(\mathbf{z}_{1:t-1}|\mathbf{x}_{1:t-1})$ and the gradient computation, and use the reparameterization trick to further lower the variance for second expectation. Furthermore, the second part of the gradient is unbiased %by reparameterization trick 

%\noindent
But, the same trick cannot be applied to $\triangledown_{\boldtheta} \mathcal{L}_t^K$, since it is not possible to drop the dependence on $\boldtheta$ %as $\triangledown_{\boldphi} \mathcal{L}_t^K$ 
unless we have the true posterior $p(\mathbf{z}_{1:t-1}|\mathbf{x}_{1:t-1})$ or the ability to draw samples from it. % There are a few ways to mitigate the high variance of gradient estimation in general \citep{mnih2014neural, mohamed2019monte, caterini2018hamiltonian, tucker2018doubly}. 
We use the score function of $p(\mathbf{x}_{t}|\mathbf{x}_{1:t-1})$ to estimate $\triangledown_{\boldtheta} \mathcal{L}_t^K$ instead:
\begin{equation}
    \begin{aligned}
        \triangledown_{\boldtheta} \mathcal{L}_t^K \simeq \sum_{i=1}^K \Tilde{w}^i_t \triangledown_{\boldtheta} \log p_{\boldtheta}(\mathbf{x}_{t}, \hat{\mathbf{z}}_{t}^{i}|\mathbf{x}_{1:t-1}, \hat{\mathbf{z}}_{1:t-1}^{i}),
    \end{aligned}
    \label{eq:gradient_theta_rws}
\end{equation}
\begin{comment}
\begin{equation}
    \begin{aligned}
        \triangledown_{\boldtheta} \log p_{\boldtheta}(\mathbf{x}_{1:T}) & = \int p_{\mathbf{\theta}}(\mathbf{z}_{1:T}|\mathbf{x}_{1:T}) \triangledown_{\mathbf{\theta}} \log p_{\mathbf{\theta}}(\mathbf{x}_{1:T}, \mathbf{z}_{1:T})  d \mathbf{z}_{1:T}\\
        & \simeq \sum_{t=1}^T \sum_{i=1}^K \Tilde{w}^i_t (\triangledown_{\boldtheta} \log p_{\boldtheta}(\mathbf{x}_{t}| \mathbf{z}_{t}^{i})+\triangledown_{\boldtheta} \log p_{\boldtheta}(\mathbf{z}_{t}^{i}| \mathbf{z}_{1:t-1}^{i})),
    \end{aligned}
    \label{eq:gradient_theta_rws}
\end{equation}
\end{comment}
\noindent
where $\hat{\mathbf{z}}_{1:T}^{i}$ are particles from samplers e.g. SMC, and $\Tilde{w}^i_t$ are normalized importance weights of $\hat{\mathbf{z}}_{1:t}^{i}$; see Appendix \ref{sec:appendix_gradient_theta_rws} for details. Essentially, the score function estimate is the same as dropping the high variance term in $\triangledown_{\boldtheta} \mathcal{L}_t^K$. Reweighted Wake-Sleep algorithm (RWS) \citep{bornschein2014reweighted} and NASMC \citep{gu2015neural} discuss a similar derivation for maximum likelihood learning. Learning by MCFOs is closely related to RWS and NASMC in terms of $\triangledown_{\boldtheta}$. However, note that the sleep phase q-update in RWS and NASMC both minimize the approximated inclusive KL-divergence, $\text{KL}(p_{\boldtheta}(\mathbf{z}_{1:t}|\mathbf{x}_{1:t})||q_{\boldphi}(\mathbf{z}_{1:t}|\mathbf{x}_{1:t}))$, by SMC, while for MCFOs the 
%MCFOs are to minimize 
disclusive KL-divergence, $\text{KL}(Q_t^K(\mathbf{z}_{1:t}^{1:K}|\mathbf{x}_{1:t})||p_{\boldtheta}(\mathbf{z}_{1:t}^{1:K}|\mathbf{x}_{1:t}))$
is minimized on the extended variable space. When the family of proposals is adequately flexible to include the true posterior $p_{\boldtheta}(\mathbf{z}_{1:t}|\mathbf{x}_{1:t})$, both RWS/NASMC and MCFOs could converge to the same optimum. However, fitting a potentially complex multi-modal posterior using a simple family of distributions
leads to undesired low density in the wide area that impairs 
%of distributions for proposal ends up with undesired low density everywhere to impair
the sample efficiency of estimators. For MCFOs, $Q_t^K(\mathbf{z}_{1:t}^{1:K}|\mathbf{x}_{1:t})$ is a mixture of simple proposals $q_{\phi}$, which remains flexible, but keeps the sample efficiency.

%\noindent
Furthermore, if the latent and observation variables of generative models are assumed to be finite-order Markovian, that they are only dependent on finite components of history, then both gradients of MCFOs could be updated by only maintaining necessary sample trajectories. Therefore, it is well suited to handle arbitrarily long sequences without memory concerns and extend to online training.

==> relatedwork.tex <==
\subsection{Monte Carlo Objectives}
\label{sec:mco}
Considering a generative model that is composed of observation $\mathbf{x}$ and latent state $\mathbf{z}$, a Monte Carlo objective (MCO) \citep{mnih2016variational} is defined as an estimate of the marginal log-likelihood $\log p(\mathbf{x})$ by samples drawn from a proposal distribution $q$. The MCO is a lower bound of $\log p(\mathbf{x})$ as given by Jensen's inequality:\vspace{-1mm}
%joint likelihood  could be considered as \textit{unnormalized} distribution $\Tilde{P}$, inference of latent variable $p(\mathbf{x}|\mathbf{z})$ as \textit{normalized} distribution, $P$, and marginal distribution  $p(\mathbf{x})$ is  normalization constant.
\begin{equation}
    \mathbb{E}_{q(\mathbf{z})}[\log R] =  \log p(\mathbf{x}) - \mathbb{E}_{q(\mathbf{z})}[\log \frac{p(\mathbf{x})}{R}],
    \label{eq:stochastic_bound}
\end{equation}
for any unbiased estimator $R$ of $p(\mathbf{x})$, that is $\mathbb{E}[R] = p(\mathbf{x})$. When an estimator takes a single sample from $q$ and $R = {p(\mathbf{x}, \mathbf{z})}/{q(\mathbf{z})}$, the MCO %is known as the Evidence Lower Bounds (ELBOs) in variational inference.
can be identified as ELBO in variational inference \citep{mnih2014neural}. When an estimator averages importance weights of $K$ samples as $R^K=K^{-1}\sum_{i=1}^K {p(\mathbf{z}^i, \mathbf{x})}/{q(\mathbf{z}^i)}$, %R_K = \frac{1}{K}\sum_{i=1}^K \frac{p(\mathbf{z}^i, \mathbf{x})}{q(\mathbf{z}^i)}$. 
, it yields an importance weighted ELBO (IW-ELBO) \citep{burda2015importance, domke2018importance}.
This bound is proven to be tighter with larger $K$ and converges to $\log p(\mathbf{x})$, as $K\rightarrow \infty$ \cite{burda2015importance}. 

\subsection{Sequential Monte Carlo}
\label{sec:smc}
For a sequential observation $\mathbf{x}_{1:T}$ with latent trajectory $\mathbf{z}_{1:T}$, a generative process %of the observation
can be factorized as $p(\mathbf{z}_{1:T}, \mathbf{x}_{1:T}) = p(\mathbf{z}_1)p(\mathbf{x}_1|\mathbf{z}_1) \prod_{t=2}^T p(\mathbf{z}_{t}|\mathbf{z}_{1:t-1}, \mathbf{x}_{1:t-1}) p(\mathbf{x}_{t}|\mathbf{z}_{1:t}, \mathbf{x}_{1:t-1})$. Inference of the latent trajectory, $p(\mathbf{z}_{1:T}|\mathbf{x}_{1:T})$ is of importance for marginalization and learning of generative models, however, it is usually intractable. 

SMC \citep{doucet2009tutorial} is a method for approximating a series of target distributions, specifically $p(\mathbf{z}_{1:T}|\mathbf{x}_{1:T})$, %for the generative model
using a set of weighted sample trajectories $\{ \Tilde{w}_{1:T}^{i}, \hat{\mathbf{z}}_{1:T}^{i} \}^{i=1:K}$. It combines Sequential Importance Sampling (SIS) and resampling, and consists of four main steps: 
\begin{itemize}
    \item[] \textit{Sample} $K$ particles $\hat{\mathbf{z}}^{i}_t$ from proposal $q(\mathbf{z}_t|\bar{\mathbf{z}}^{i}_{1:t-1},\mathbf{x}_{1:t})$ with previous resampling trajectories $\bar{\mathbf{z}}^{i}_{1:t-1}$;
    \item[] \textit{Append} $\hat{\mathbf{z}}^{i}_{1:t}=(\hat{\mathbf{z}}^{i}_t, \bar{\mathbf{z}}^{i}_{1:t-1})$; 
    \item[] \textit{Weight} $w_t^{i} = {p(\mathbf{x}_{1:t}, \hat{\mathbf{z}}_{1:t}^{i}|\mathbf{x}_{1:t-1}, \bar{\mathbf{z}}^{i}_{1:t-1})}/{q(\hat{\mathbf{z}}^{i}_t|\bar{\mathbf{z}}^{i}_{1:t-1},\mathbf{x}_{1:t})}$, $\Tilde{w}_t^{i}={w_t^{i}}/{\sum_{j=1}^K w_t^{j}}$;
    \item[] \textit{Resample} $\{\Tilde{w}_t^{i}, \hat{\mathbf{z}}_{1:t}^{i} \}$ to obtain equally-weighted particles $\{\frac{1}{K}, \bar{\mathbf{z}}^{i}_{1:t}\}$.
\end{itemize}
This iteration continues until time step T; see Algorithm \ref{algo:SMC} in Appendix \ref{sec:appendix_smc} for details of SMC. Besides being considered as an approximate inference, SMC also gives an unbiased estimate of marginal likelihood $p(\mathbf{x}_{1:T})$ by importance weights:
\begin{equation}
    \hat{p}(\mathbf{x}_{1:T}) = \prod_{t=1}^T \left( \frac{1}{K} \sum_{i=1}^K w_t^i \right).
    \label{eq:smc_estimator}
\end{equation}
Compared to SIS, although resampling increases the intermediate variance, it resolves the \textit{degeneracy} problem that occurs when only a single or few trajectories dominate, therefore, impairing the total variance of the whole sequence. The sample efficiency of SMC is largely dependent on the choice of proposal distributions and it is usually difficult to scale up SMC to higher dimensions due to inefficient approximation of complex posterior distributions. %We refer to Appendix \ref{sec:appendix_smc} and \citep{doucet2009tutorial} for more in-depth discussion on SMC.


\subsection{Variational Filtering Objectives}
As mentioned in the introduction, various ELBO-like surrogate objectives have been proposed to learn generative sequence models, %such as STONE \citep{bayer2014learning}, VRNN \citep{chung2015recurrent}, SRNN \citep{fraccaro2016sequential}, DKF \citep{karl2016deep}, KVAE \citep{fraccaro2017disentangled} and AVF \citep{marino2018general}, 
% ALREADY MENTIONED
using different factorizations of generative models and structural approximations of variational (proposal) distributions. IWAE \citep{burda2015importance} could be extended from Importance Sampling (IS) to SIS by defining an estimator $R^K=K^{-1}\sum_{i=1}^K {p(\mathbf{z}_{1:T}^i, \mathbf{x}_{1:T})}/{q(\mathbf{z}_{1:T}^i)}$. However, such an estimator suffers from the aforementioned high variance degeneracy of SIS. To improve this, AESMC \citep{le2017auto}, VSMC \citep{naesseth2018variational} and FIVO \citep{maddison2017filtering}, three closely related MCOs, apply estimators defined by SMC as in (\ref{eq:smc_estimator}). The main differences between these objectives lie in the implementation of SMCs: AESMC implements the classic SMC \citep[Section~3.5]{doucet2009tutorial}; VSMC assumes Markovian latent variables and conditional independence of observation so that proposals and conditionals in the generative model are simplified; FIVO defines its objective by adaptive resampling SMC \citep[Section~3.5]{doucet2009tutorial}, but learns with the fixed schedule of resampling as AESMC. 

In the following section, we propose MCFOs, a family of variational filtering objectives, inspired by MCOs and FIVOs. We examine their important properties and discuss the choice of importance proposal on the tightness of MCFOs and their relations to previous objectives and how to optimize MCFOs to learn parametric generative and adaptive proposal models from data.
